Too Brittle To Touch: Comparing the Stability of Quantization and Distillation Towards Developing Lightweight Low-Resource MT Models

Leveraging shared learning through Massively Multilingual Models, state-of-the-art machine translation models are often able to adapt to the paucity of data for low-resource languages. However, this performance comes at the cost of significantly bloated models which are not practically deployable. Knowledge Distillation is one popular technique to develop competitive, lightweight models: In this work, we first evaluate its use to compress MT models focusing on languages with extremely limited training data. Through our analysis across 8 languages, we find that the variance in the performance of the distilled models due to their dependence on priors including the amount of synthetic data used for distillation, the student architecture, training hyperparameters and confidence of the teacher models, makes distillation a brittle compression mechanism. To mitigate this, we explore the use of post-training quantization for the compression of these models. Here, we find that while distillation provides gains across some low-resource languages, quantization provides more consistent performance trends for the entire range of languages, especially the lowest-resource languages in our target set.

==> background.tex <==

\section{Background}

\begin{table*}[!h]
    \centering
    \small
    \begin{tabular}{ccccccc}
        \toprule
        \multirow{2}{*}{Language} & \multicolumn{2}{c}{Data Constraints} & \multicolumn{2}{c}{Model Constraints} \\
        %\cline{2-5}
        & Monolingual Data & Parallel Data & Seen/Shared Script with HRL & Included in Pretraining  \\
         \midrule
         Bribi & \scalecross & \scalecheck & \scalecross & \scalecross  \\
         Wixarica & \scalecross & \scalecheck & \scalecross & \scalecross  \\
         Mundari & \scalecross & \scalecheck & \scalecheck & \scalecross  \\
         Gondi & \scalecross & \scalecheck & \scalecheck & \scalecross  \\
         Assammese & \scalecheck & \scalecheck & \scalecheck & \scalecheck \\
         Odia & \scalecheck & \scalecheck & \scalecross & \scalecross \\
         Punjabi & \scalecheck & \scalecheck & \scalecross & \scalecheck \\
         Gujarati & \scalecheck & \scalecheck & \scalecross & \scalecheck \\
         \bottomrule
    \end{tabular}
    \caption{Languages Under Consideration: Note that the except the language's inclusion in the pretraining corpus of our chosen pretrained language models, all factors are independent of our experimental setup. }
    \label{tab:languages}
\end{table*}


For the purpose of our work we expect that the compressed variant of any given model, \currentmodel, should at least fulfill the following two conditions:  
\begin{enumerate}
    \item \currentmodel should \textbf{achieve some measurable size reduction over a the highest-performing model} possible for the given language. 
    
    % We further constraint the size of the compressed model to be under an \edgesize. This threshold size can be expected to be a representative of an edge-device induced constraints that would limit the deployment of any model larger than the \edgesize. We fix the \edgesize as \textit{500 MB} works for this work. For reference the chosen \edgesize is expected to operate reasonably well for a model that is expected to be deployed across an edge-device operating with Android 5 or higher versions for devices with a minimum on-device RAM of 2GB.  \footnote{Google Play Store Reference}.
    
    
    \item \textbf{\currentmodel has to perform reasonably well}: The accuracy gap between highest-performing model in that language and the \currentmodel should be minimum. 
\end{enumerate}

\noindent 
Let $\size(\currentmodel)$ denote the size of \currentmodel and let the highest-performing\footnote{Note that for the purpose of this work, the highest performing model is synonymous to a strong baseline model} model (denoted by \bestmodel for brevity) over a family of models for a given language be defined as: 
\begin{align}
    \bestmodel = \argmax_{\givenmodel \in \currentmodels} \acc(\givenmodel) \nonumber
\end{align}

\noindent Then to measure the compressed model's affinity to compression we define a simple metric that reconciles the above stated requirements. Note that this metric is only used improve readability of our experimental analysis. 

%  quantifies the gap in performance between \currentmodel and the \textit{highest-performing model}, \bestmodel, available for that language, as well as the size threshold that exists for a any given edge platform. Concretely, we define the metric as: 

\begin{align}
    \modelreadiness(\givenmodel) = \left(\frac{\acc(\bestmodel)-\acc(\givenmodel))}{\acc(\bestmodel)}\right) \frac{\size(\givenmodel)}{\edgesize} 
\end{align}


% \subsection{Interpretation of \modelreadiness}

% A deployment gap of 0 indicates the availability of immediately deployable systems \textit{or} The lesser the \modelreadiness, the lesser is the gap between the \bestmodel and the \currentmodel across the two dimensions of consideration - Performance and Size. This is because either the first term (performance gap between \givenmodel and \bestmodel) decreases or the second term (size) of the model decreased. Note, that if $\size(\givenmodel)$ is greater than \edgesize, the model cannot be deployed and \modelreadiness is set as 1. 
